Subject Data Auditing via Source Inference Attack in Cross-Silo Federated Learning

Source Inference Attack (SIA) in Federated Learning (FL) aims to identify which client used a target data point for local model training. It allows the central server to audit clients' data usage. In cross-silo FL, a client (silo) collects data from multiple subjects (e.g., individuals, writers, or devices), posing a risk of subject information leakage. Subject Membership Inference Attack (SMIA) targets this scenario and attempts to infer whether any client utilizes data points from a target subject in cross-silo FL. However, existing results on SMIA are limited and based on strong assumptions on the attack scenario. Therefore, we propose a Subject-Level Source Inference Attack (SLSIA) by removing critical constraints that only one client can use a target data point in SIA and imprecise detection of clients utilizing target subject data in SMIA. The attacker, positioned on the server side, controls a target data source and aims to detect all clients using data points from the target subject. Our strategy leverages a binary attack classifier to predict whether the embeddings returned by a local model on test data from the target subject include unique patterns that indicate a client trains the model with data from that subject. To achieve this, the attacker locally pre-trains models using data derived from the target subject and then leverages them to build a training set for the binary attack classifier. Our SLSIA significantly outperforms previous methods on three datasets. Specifically, SLSIA achieves a maximum average accuracy of 0.88 over 50 target subjects. Analyzing embedding distribution and input feature distance shows that datasets with sparse subjects are more susceptible to our attack. Finally, we propose to defend our SLSIA using item-level and subject-level differential privacy mechanisms.

==> sections/related_work.tex <==
\section{Related Works}

\subsection{Privacy and Security Attacks in Federated Learning}

Shokri et al.~\cite{Shokri_2015_Privacy} propose the collaborative learning DSSGD, a privacy-preserving strategy, to avoid the central collection of private data for model training and maintain the performance on the task. In their framework, the local clients train their models, upload the gradients of partial parameters to the central server for aggregation, and update partial local parameters with the global model. Phong et al.~\cite{Phong_2017_HE_on_FL} show an honest but curious server can extract the training data from partial gradients uploaded by the local client in the framework of Shokri et al. Specifically, they observe that the division between the gradient on the weight and bias is related to one specific input value (like one image pixel), making extracting the input value from the gradient feasible if the training batch has only one data point. Hence, they propose to encrypt uploaded gradients with additively holomorphic encryption and maintain the consistency of operation over the encrypted gradients, which prevents privacy leakage from the server. Hitaj et al.~\cite{Hitaj_GAN_2017} implement a GAN-based reconstruction attack, which generates the images belonging to the label the adversary (a malicious federation user) does not hold. Specifically, the adversary trains a local GAN to generate images whose label is in a victim user by utilizing the global model as the discriminator and mislabeling the generated images as the label the adversary holds, which makes the victim user reveal more information about the target label of the adversary. Wang et al.~\cite{Wang_2019_User_level} propose an extract data reconstruction against the victim client from the perspective of the central server without disrupting the federated learning via training a GAN with a multi-task discriminator, which distinguishes not only fake and real images but also different categories and identity information (from victim client or other clients). With the GAN, the server can generate data (labeled with a specific category) from the victim client. 

Zhu et al.~\cite{Zhu_2019_Deep_leakage} recover the training data and labels of local clients by the iterative update of dummy inputs and labels to match the gradient update via L-BFGS~\cite{Dong_1989_LBFGS}, which works well if a single pair of input and label in the batch. For more data points in the batch, they reconstruct each by calculating the gradient separately. Considering the inconsistency of convergence and discovering ground-truth labels in~\cite{Zhu_2019_Deep_leakage}, Zhao et al.~\cite{zhao_2020_idlg} propose a reliable method to extract ground-truth labels from shared gradients via observing the signs of gradients on the parameters of the last layer. Under the one-hot encoding and cross-entropy loss, the loss gradient on the logit of the ground-truth label is negative. In contrast, gradients on other labels' logits are positive, exposing the ground-truth labels. With the weights of the last layer, the weight with a different gradient from other weights is for the ground-truth label by analyzing the relation between the gradients of the logit and the weight of the last layer. With the ground-truth labels, the reconstruction is more stable and efficient. Geiping et al.~\cite{Geiping_2020_invert_gradient} utilize Adam~\cite{Adam_Diederik_2015} to optimize a cosine similarity with a regularization term about the total variation of the input to align the gradient updates of original and reconstructed inputs instead of a euclidean loss optimized with L-BFGS~\cite{Dong_1989_LBFGS} in previous works~\cite{Zhu_2019_Deep_leakage,zhao_2020_idlg}. 

Melis et al.~\cite{melis_2019_exploiting} infer the membership of a text or location in other clients by checking whether the embedding weights of its tokens are all non-zero in the aggregated embedding layer of arbitrary training epoch from a malicious client. For the passive property inference, they calculate batch gradients of the global model on the auxiliary data with and without the specific property to train a binary classifier to predict whether a batch holds this property. Besides, they combine the main task with a batch property classifier via multi-task learning in the local training of the adversary to achieve the active property inference. Nasr et al.~\cite{nasr_2019_comprehensive} extend the black-box membership inference attack with activation outputs of the model under white-box condition, which is not better than the black-box one. Hence, they utilize the gradients of all parameters on the target data point as the primary attack feature. Besides, the adversary can push the SGD to leak more information by applying the gradient ascent on target data points before uploading it to the central server or sending it to local users. They cluster the gradient embeddings with unsupervised learning for membership prediction instead of training a binary classifier with shadow model strategy like the previous non-FL scenario~\cite{shokri_membership_2017} if the adversary does not hold data points from the training data. Zari et al~\cite{zari_2021_efficient} reduce the heavy feature of the attack model in~\cite{nasr_2019_comprehensive} by combining the outputs of models from the target client on the ground-truth label among training rounds as the feature of the attack model. Gu et al.~\cite{Gu_2022_CSMIA} observe the prediction confidence of training data rises faster than testing data among FL rounds. They measure the prediction confidence with the prediction probability of the ground truth label and the modified prediction entropy~\cite{song_systematic_2021}. Their strategies are based on the shadow model~\cite{shokri_membership_2017} with data whose membership is known for extracting the dataset for training a binary attack model. As one adversary user of FL, they regard the local model as the shadow model. Being the central server, they propose a passive method to fine-tune a shadow model with the auxiliary data and aggregate it with the global model as the new shadow model without disturbing the standard FL. Besides, they put forward an active approach to train a shadow model with the auxiliary data as one of the local clients to update with the global model together. Li et al.~\cite{li2023effective} observe that gradients of different data points in the training data are nearly orthogonal under an overparameterized model trained with enough epochs. Based on this, they propose calculating the cosine similarity between the gradient of the target data point and the sum of gradients uploaded by the local client. If the target data point is in the training data of the local client, the cosine similarity should be around one. They also compare the L2 norm of the sum of gradients and the one subtracting the target data point's gradient. If the gap of the L2 norm is greater than zero, they predict the target data point is in the training data. Zhang et al.~\cite{Zhang_2023_efficient_MIA} propose using the model's biases rather than weights for the membership inference attack. For a target data point, they concatenate the changes of biases (last layer) between neighboring models among selected global models as the feature to predict membership from the perspective of a local user. As the central server, they observe the bias changes of the data point from all local users in multiple epochs. Then, they determine the user with more times to obtain a minor bias change of the data point among epochs as the source, which means that the data point is in the training data of this user. Pichler et al.~\cite{pichler2022perfectly} implement a perfectly accurate membership inference attack by inserting an intentionally designed network into the local client and observing a bias change magnitude to predict membership from the perspective of a dishonest central server.

Zhang et al.~\cite{Zhang_2022_GANMIA} implement a passive membership inference attack from the perspective of one participant by training a GAN to generate data points close to the training data of the target FL model, which enriches member data points diversity of training the attack model. The discriminator of the GAN is initialized with the target FL model to predict whether the data point is from the original training data. As the participant has a set of data points from the original training data, he can update the discriminator and generator with the original and generated data via adversarial training to make the generated data close to the training data. With original and generated data as the member data and some test data as non-member data, they will train an attack model to predict the membership for each category in the target FL model using the data from the specific label. Chen et al.~\cite{Chen_user-level_2020} propose a user-level membership inference attack to infer whether the data is from one victim client from the perspective of another client, assuming all clients do not share identical labels. They locally train a GAN with the global model as the discriminator to gradually generate data points close to real ones from all labels via adversarial training. With generated data points, they train an attack model with the task of label classification. If the attack model correctly predicts a data point whose label is in the labels of the victim client, it indicates this data point is in the training data of the victim client. In their extensive work~\cite{Zhao_user-level_2021}, they isolate the updated model from the victim client and train a GAN to generate data points close to the training data of the victim client by only mutually updating the discriminator and the local model of the victim client from the perspective of the central server. They predict the labels of generated data with the aggregated global model, combine other data from other clients to train an attack model as a label classifier for predicted label comparison, and infer a data point is from the victim client if its label is in the labels of the victim client.
% \subsection{Security Attacks in Federated Learning}

\subsection{Property inference attack}

Ateniese et al.~\cite{Ateniese_2015_Hacking} extract features (e.g., the support vectors of SVM) from the target model to predict the property of its training data via training a set of shadow classifiers, half of whose training data holds the property. For neural networks, Ganju et al.~\cite{Ganju_2018_PIA} infer sensitive global properties of the training data by taking all the parameters of a neural network
as the feature representation. To reduce the impact of permutation-equivalent networks, they propose to sort the neuron weights or regard them as a set. Instead of obtaining inference signals from the model parameters, Zhang et al.~\cite{zhang2021leakage} infer the distribution of a sensitive attribute in the training data of the target model via querying the target model and concatenating the posterior probability vectors of data points from an attack dataset to construct the feature for the property inference. Similarly, they train shadow models with and without the property for querying with the attack dataset to extract concatenated probabilities for training the meta-classifier. Mahloujifar et al.~\cite{Mahloujifar_2022_PIA_from_poisoning} explore whether the poisoning attack will enlarge the information leakage measured with the property inference attack. Suri et al.~\cite{suri2022formalizing} formulate the property and attribute attacks as the distribution inference attack and extend the meta-classifier in ~\cite{Ganju_2018_PIA} to convolutional neural networks via concatenating the kernel weight matrix along the input channel dimension to obtain a similar format of weights like a linear layer. Besides, they propose two black-box methods: the loss test compares the prediction accuracy of data sampled from two candidate distributions, and the threshold test uses trained models to derive a threshold on observed accuracy on the data sample (from one of the distribution), which maximizes the accuracy gap between models with and without the property, for determining the distribution of the target model. In their subsequent work~\cite{Suri_2023_DIA}, they propose a black-box property inference attack by comparing the probability distribution of a set of data (half with the property and half not) between the target model and each pair of shadow models (one is trained with the data holding property and the other not) via calculating the KL-divergence value. Suppose the probability distribution is close to the ones obtained from the shadow models trained with the data holding the property. In that case, they predict the target model holds the property and vice versa. Hartmann et al.\cite{Hartmann_2023_DIA} analyze the reasons for distribution leakage, including the label difference for the same feature within two distributions and imperfect models caused by the wrong inductive bias and finite training data. They propose to reduce the leakage according to reasons and utilize causal learning (invariant risk minimization~\cite{arjovsky2019invariant}) to eliminate the distributional membership inference.

%Specifically, they sample poisoning data points to compensate for the training data of the shadow models, and the rate of training data that holds the property is selected from two rates. With the query set, the adversary trains a model to distinguish those two rates by querying the shadow models. 

% However, they need to train an equal number of shadow classifiers as the number of data points for teaching the attack model (meta-classifier), which requires more computation resources. Besides, those two methods are designed for general properties like the voice accent, skin color, and age rather than including data points from a specific subject, which is an inconspicuous property. 

\subsection{Source Inference and Subject Membership Inference Attacks}

Hu et al.~\cite{SIA_Hu} propose the source inference attack, which aims to detect the client trained with one specific data point in Federated Learning, assuming this data point is in the training data of only one client. Their strategy is calculating the losses of this data point on all clients and predicting the client with the lowest loss on this data point as the client trains with it from the perspective of a curious but honest central serve in Federated Learning. There are two drawbacks to their work. One is that they assume that only one client trains its local model with the target data point, ignoring the scenarios that none or more than one client prepares local models with this data point, which is infeasible with their strategy. Besides, instead of holding a target data point in clients' training data to investigate the source, the central sever cares more about whether the data from a specific subject is used for local training and where the data is used without knowing which data is used. This task is similar to a subject membership inference attack proposed by Suri et al.~\cite{suri2022subject}. The subject membership inference attack infers whether any client trains its local model with data points from the target subject in cross-silo Federated Learning. Each client might prepare its local model with data points from multiple subjects, such as handwriting digital numbers from different writers for the local digital number recognition task. They put forward the Loss-Threshold attack, which counts the data points from the target subject with a lower loss than a threshold, and the Loss-Across-Rounds attack, which measures the number of decreases of the loss accumulated with the data points of the target subject among the training epochs to determine whether any clients train with the data from the target subject. They audit whether the data from the target subject utilizes the data not used for training. However, they can not precisely distinguish which client trains its local model with the data from the target subject.

Liu et al.~\cite{Liu_23_SubjectMIA} investigate the subject-level membership inference attack on a group of interested federation users. Given a data point of the target subject, they aim to predict whether any concerned users use the data from the same subject as the data point. The adversary trains a GAN during the FL training to perform data augmentation on a few known data. Specifically, the adversary acts as a regular user to download the global model to reparameterize the discriminator model of the GAN and utilize the adversarial training to make the generator generate data points whose subjects are in and not in the training data of concerned users. With more data, they train a classifier with the combined posteriors of the aggregated model of concerned users and the global model on a data point as the feature to distinguish whether any data from the subject of this data point is in the training data of concerned users. There are some strong assumptions about their work. The first is that the adversary holds 10\% data points of each subject in the training data of concerned users. Second, they can not exactly figure out all the users who train their local models with the data from a specific subject in FL as they care about a group of users. Third, the adversary can interrupt the FL training by uploading the trained discriminator model to the server. Besides, they do not use the dataset with a concept of subject for evaluation but model each subject as a parametric distribution using a multivariate Gaussian distribution.
